Pushing the performances of ASR models on English and Spanish accents

Speech to text models tend to be trained and evaluated against a single target accent. This is especially true for English for which native speakers from the United States became the main benchmark. In this work, we are going to show how two simple methods: pre-trained embeddings and auxiliary classification losses can improve the performance of ASR systems. We are looking for upgrades as universal as possible and therefore we will explore their impact on several models architectures and several languages.

==> tables/accentDataDistribution.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
    \toprule
      Accent & Duration(hours)\\
      \midrule
      es\_ar [Argentina] & 19 \\
      es\_es [Spain] & 23 \\ 
      es\_gt [Guatemala] & 24 \\
      es\_pe [Peru] & 24 \\ 
      es\_ve [Venezuela] & 24 \\ 
      es\_latam [all Latin America] & 35 \\
    \bottomrule
    \end{tabular}
    \caption{
      \textbf{Duration (hours) per accent to benchmark models trained with UsageSpanish}
    \label{tab:UsageSpanishAccents}}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
    \toprule
      Accent & Duration (hours)\\
      \midrule
      en\_co [Columbia] & x.xx \\
      en\_eg [Egypt] & x.xx \\
      en\_mm [Myanmar] & x.xx \\ 
      en\_nz [New Zealand] & x.xx \\
      en\_pk [Pakistan] & x.xx \\
      en\_br [Brazil] & x.xx \\ 
      en\_de [Germany] & x.xx \\ 
      en\_ru [Russia] & x.xx \\
      en\_tw [Taiwan] & x.xx \\
      en\_ph [Philippines] & x.xx \\
      en\_mx [Mexico] & x.xx \\ 
      en\_sq [Scotland] & x.xx \\
      en\_it [Italy] & x.xx \\
      en\_fr [France] & x.xx \\ 
      en\_kr [Korea] & x.xx \\ 
      en\_vn [Vietnam] & x.xx \\
      en\_ca [Canada] & x.xx \\
      en\_gb [UK] & x.xx \\
      en\_ar [Argentina] & x.xx \\ 
      en\_bd [Bangladesh] & x.xx \\
      en\_en [England] & x.xx \\
      en\_in [India] & x.xx \\ 
      en\_ng [Nigeria] & x.xx \\ 
      en\_ie [Ireland] & x.xx \\
      en\_za [South Africa] & x.xx \\
      en\_au [Australia] & x.xx \\ 
      en\_us [US] & x.xx \\
    \bottomrule
    \end{tabular}
    \caption{
      \textbf{Duration (hours) per accent to benchmark models trained with UsageEnglish}
    \label{tab:UsageEnglishAccents}}
\end{table}

==> tables/mtl_loss.tex <==
\addtolength{\tabcolsep}{-2pt} 
\begin{table}[h!]
    \centering
    \begin{tabular}{l|cccccc}
    \toprule
      Model  & \multicolumn{2}{c}{en} & \multicolumn{2}{c}{es} & \multicolumn{2}{c}{ar} \\
        & $w_{s}$ & $w_{b}$ & $w_{s}$ &$w_{b}$ & $w_{s}$ & $w_{b}$  \\
      \midrule
      w2v & x.xx & x.xx & x.xx & x.xx & x.xx & x.xx\\ 
      w2v + mtl & x.xx & x.xx & x.xx & x.xx & x.xx & x.xx\\ 
      \midrule
      cf.300 & x.xx & x.xx & x.xx & x.xx & x.xx & x.xx\\ 
      cf.300 + mtl & x.xx & x.xx & x.xx & x.xx & x.xx & x.xx\\ 
      \midrule
      prod & x.xx & x.xx & x.xx & x.xx & x.xx & x.xx\\ 
      prod + mtl & x.xx & x.xx & x.xx & x.xx & x.xx & x.xx\\ 
    \bottomrule
    \end{tabular}
    \caption{
      \textbf{WER MTL Loss}
    \label{tab:mtl}}
\end{table}
\addtolength{\tabcolsep}{2pt} 




==> tables/pre_training.tex <==
\addtolength{\tabcolsep}{-2pt} 
\begin{table}[h!]
    \centering
    \begin{tabular}{l|c|cc|cc}
    \toprule
       \multirow{2}{*}{Model}  & \multirow{2}{*}{pretr.} & \multicolumn{2}{c|}{es} & \multicolumn{2}{c}{en} \\
         & &   $w_s$ & $w_b$ & $w_s$ & $w_b$  \\
      \midrule
      \transformerbig & No & x.xx & x.xx & x.xx & x.xx\\
      \midrule
      \multirow{ 3}{*}{\shortstack[l]{\wavvec\\ 94M}}  & No & x.xx & x.xx & x.xx & x.xx \\
      &  \vphundred & x.xx & x.xx & x.xx & x.xx  \\
       &  \indomaines & x.xx & x.xx & x.xx & x.xx  \\
    \bottomrule
    \end{tabular}
    \caption{
      \textbf{Average WER per accent using embeddings pre-trained on different datasets}: $w_s$ being the smallest average wer by accent and $w_b$ the biggest one.  We compare settings without any pre-training, with  out of domain pre-training on VoxPopuli (\vphundred) and with in-domain pre-training (\indomaines). 
    \label{tab:pre_training}}
\end{table}
\addtolength{\tabcolsep}{2pt} 

==> tables/unseen_accents.tex <==
\addtolength{\tabcolsep}{-2pt} 
\begin{table}[h!]
    \centering
    \begin{tabular}{l|cc|ccc}
    \toprule
            & \multicolumn{2}{c|}{In domain} &  \multicolumn{3}{c}{Unseen accents} \\
      Model  & $w_{s}$ & $w_{b}$ & $w_{1}$ &$w_{2}$ & $w_{3}$ \\
      \midrule
      wav2vec & x.xx & x.xx & x.xx & x.xx & x.xx \\ 
      wav2vec + mtl & x.xx & x.xx & x.xx & x.xx & x.xx \\ 
      \midrule
      conf.300 & x.xx & x.xx & x.xx & x.xx & x.xx \\ 
      conf.300 + mtl & x.xx & x.xx & x.xx & x.xx & x.xx \\ 
      \midrule
      prod & x.xx & x.xx & x.xx & x.xx & x.xx \\ 
      prod + mtl & x.xx & x.xx & x.xx & x.xx & x.xx \\ 
    \bottomrule
    \end{tabular}
    \caption{
      \textbf{WER Unseen accents (english} : smallest $w_s$ and biggest $w_b$ median WER on accents observed at training time. Completing the study with the medianWER on 3 unseen accents.
    \label{tab:mtl}}
\end{table}
\addtolength{\tabcolsep}{2pt} 
